Learning Structured Compressed Sensing with Automatic Resource Allocation

Multidimensional data acquisition often requires extensive time and poses significant challenges for hardware and software regarding data storage and processing. Rather than designing a single compression matrix as in conventional compressed sensing, structured compressed sensing yields dimension-specific compression matrices, reducing the number of optimizable parameters. Recent advances in machine learning (ML) have enabled task-based supervised learning of subsampling matrices, albeit at the expense of complex downstream models. Additionally, the sampling resource allocation across dimensions is often determined in advance through heuristics. To address these challenges, we introduce Structured COmpressed Sensing with Automatic Resource Allocation (SCOSARA) with an information theory-based unsupervised learning strategy. SCOSARA adaptively distributes samples across sampling dimensions while maximizing Fisher information content. Using ultrasound localization as a case study, we compare SCOSARA to state-of-the-art ML-based and greedy search algorithms. Simulation results demonstrate that SCOSARA can produce high-quality subsampling matrices that achieve lower Cram\'er-Rao Bound values than the baselines. In addition, SCOSARA outperforms other ML-based algorithms in terms of the number of trainable parameters, computational complexity, and memory requirements while automatically choosing the number of samples per axis.

==> sec_ara.tex <==
\section{Automatic Resource Allocation}\label{sec_ara}
%\begin{itemize}
%    \item Deduction of the Gram matrix.
%    \begin{itemize}
%        \item $\bm{\phi}\rightarrow \bm{\Phi}\rightarrow \bm{\Psi}$.
%    \end{itemize}
%    \item Extract subsampling matrices.
%    \begin{itemize}
%        \item Extract $\mathbf{S}_i$ from $\bm{\Psi}$.
%    \end{itemize}
%    \item Take its trace as a regularization term.
%    \begin{itemize}
%        \item $\mathrm{Trace}(\bm{\Psi})=\Vert \bm{\Phi} \Vert_{\rm{F}}^2$
%    \end{itemize}
%    \item Scaling matrix controls compression priority.
%    \begin{itemize}
%        \item $\mathrm{Trace}(\bm{D}\bm{\Psi})$.
%    \end{itemize}
%    \item Add the updated figure to explain the process. (Maybe we can remove the algorithm pseudocode.)
%\end{itemize}

% \noindent In the Deep Probabilistic Subsampling (DPS) framework, the design of subsampling matrices is treated as the drawing of samples from categorical distributions whose log probabilities are learned by means of a softmax neural network using the Gumbel reparametrization trick \cite{jang2017categorical, maddison2017concrete}. In DPS, all axes are considered simultaneously without structure, leading to a subsampling matrix with as many degrees of freedom as samples in the data. 

\noindent Given a total sampling budget $M_\Sigma=\sum_{i=1}^{q}M_i$ and the number of dimensions $q$ in the data, the samples can be allocated in $\binom{M_{\sum} - 1}{q - 1}$ number of ways, resulting in a combinatorial resource allocation problem. Instead of heuristically specifying the active elements $M_i$ per axis, we automatically learn how to distribute the sampling budget.

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.8\textwidth, trim = {0cm 0cm 0cm 0.1cm}, clip]{fig_scosara_flowchart_new.eps}
	\caption{Flowchart of automatic resource allocation in SCOSARA. There are two parallel ways to obtain the subsampling matrices and the regularizer: the top path perturbs the logits with Gumbel noise to approximate the process of sampling from a categorical distribution, while the lower path directly uses the logits to produce the regularizer. The matrix $\bm{D}$ in the trace computation is a scaling matrix that controls the compression priority.}
	\label{fig_scosara}
    \vspace{-0.5cm}
\end{figure*}


Following the Deep Probabilistic Sampling (DPS) framework~\cite{huijben2020DPS}, we introduce a vector $\bm{\phi}$ containing $N_\Sigma=\sum_{i=1}^{q}N_i$ unnormalized log-probabilities (or `logits') that represent the probabilities of selecting the respective elements from $\mathbf{y}$. 
From this vector, a total of $M_\Sigma$ samples are drawn without replacement, which generates a selection of $M_\Sigma$ samples across the $q$ compression axes. As illustrated in Figure \ref{fig_scosara}, one initializes a logits vector $\bm{\phi} \in \real^{N_\Sigma}$ and adds Gumbel noise to form the perturbed logits vector $\tilde{\bm{\phi}}$. We then repeat the vector $M_\Sigma$ times and apply a softmax to form an auxiliary matrix $\tilde{\bm{\Phi}} \in \real^{M_\Sigma\times N_\Sigma}$ which contains the per-axis subsampling matrices, as well as nuisance entries. This matrix then goes into two parallel computation graphs: one for the $\topK-\softmax$ \cite{huijben2020DPS} processing and the other for the regularization term. 

For the $\topK-\softmax$ processing, after applying $\topK$ to extract the indices of $M_\Sigma$ largest values in $\tilde{\bm{\phi}}$, we need to construct a mask matrix $\bm{W}\in \real^{M_\Sigma\times N_\Sigma}$. At the $i$th row of $\bm{W}$ ($i=1, \dots, M_\Sigma$), the positions of the previous $(i-1)$ largest values should be set to $-\infty$, which ensures that the largest position of rows will not be repeatedly selected after the row-wise $\softmax$ operation.

%Two challenges arise here. First, the matrix $\bm{\Phi}$ contains extraneous entries that don't fit into any of these matrices. Second, because all axes are pooled together and samples are drawn randomly, it is not known a priori which rows of $\bm{\Phi}$ correspond to which axis.

The compression matrices can be systematically obtained as follows. The $q$-dimensional data array $\mathbf{Y}$ is first column-wise vectorized, noting that the vectorization order determines the order in which the subsampling matrices $\mathbf{S}_i$ appear in $\tilde{\boldsymbol{\Phi}}$. The first $M_1$ rows and $N_1$ columns of $\tilde{\boldsymbol{\Phi}}$ represent the subsampling of the first data acquisition dimension, the next $M_2$ rows and $N_2$ columns represent the second dimension, and so forth. Thus, we have
\begin{align}
	\label{eq_phihat}
	\tilde{\bm{\Phi}}=
	\begin{bmatrix}
		\mathbf{S}_1 & \mathbf{N}_{1,2} & \cdots & \mathbf{N}_{1,q} \\
		\mathbf{N}_{2,1} & \mathbf{S}_2 & \cdots & \mathbf{N}_{2,q} \\
        \vdots & \vdots & \ddots & \vdots \\
		\mathbf{N}_{q,1} & \mathbf{N}_{q,2} & \cdots & \mathbf{S}_q
	\end{bmatrix},
\end{align}
where the off-diagonal blocks $\mathbf{N}_{i,j} \in \real^{M_i \times N_j}, 1 \leq i,j \leq q$, contain only nuisance terms due to the rows of $\tilde{\boldsymbol{\Phi}}$ being approximately one-hot, and $\mathbf{S}_i \in \real^{M_i \times N_i}$. 

In the DPS framework, since the logits are updated iteratively and perturbed with Gumbel noise, we instead obtain $\bm{\Pi} \tilde{\bm{\Phi}}$, where $\bm{\Pi} \in \mathbb{R}^{M_\Sigma \times M_\Sigma}$ is an unknown permutation matrix. The permutation matrix can be removed by computing $\bm{\Psi} = (\bm{\Pi} \tilde{\bm{\Phi}})^\mathrm{T} (\bm{\Pi} \tilde{\bm{\Phi}}) = \tilde{\bm{\Phi}}\trans \tilde{\bm{\Phi}} \in \mathbb{R}^{N_\Sigma \times N_\Sigma}$, yielding a matrix of the general form
%\vspace{-0.5\baselineskip}
\begin{align}
	\label{eq_psi}
	{\bm{\Psi}}=
	\begin{bmatrix}
		\mathbf{S}_1\trans \mathbf{S}_1 + \mathbf{N}'_{1}  & \mathbf{N}'_{1,2} & \cdots & \mathbf{N}'_{1,q} \\
		\mathbf{N}'_{2,1} & \mathbf{S}_2\trans \mathbf{S}_2 + \mathbf{N}'_{2} & \cdots & \mathbf{N}'_{2,q} \\
        \vdots & \vdots & \ddots & \vdots \\
		\mathbf{N}'_{q,1} & \mathbf{N}'_{q,2} & \cdots & \mathbf{S}_q\trans \mathbf{S}_q + \mathbf{N}'_{q}
	\end{bmatrix}.
\end{align}
The block matrices along the diagonal of $\bm{\Psi}$, $\tilde{\mathbf{S}}_1 = \mathbf{S}_1^\mathrm{T} \mathbf{S}_1 + \mathbf{N}'_{1} \in \real^{N_1 \times N_1}$ and similarly for the others, can then be used to construct
\begin{align}
\vspace{-0.4cm}
	\label{eq_subsamp}
	\tilde{\mathbf{S}} = \tilde{\mathbf{S}}_1 \otimes \tilde{\mathbf{S}}_2 \otimes \cdots \otimes \tilde{\mathbf{S}}_q \in \real^{N_\Pi \times N_\Pi}.
\vspace{-0.4cm}
\end{align}

Since the rows of $\tilde{\bm{\Phi}}$ are non-negative and sum to one due to the $\softmax$ function, maximizing $\mathrm{Trace}(\bm{\Psi})$ (equivalently, $\|\tilde{\bm{\Phi}}\|_\mathrm{F}^2$) reduces the magnitude of the off-diagonal elements and makes $\bm{\Psi}$ more like a row-wise one-hot subsampling matrix, thereby aligning the forward and backward passes of the straight-through estimator. This provides a regularization term to be added to the cost function. Furthermore, the trace can be weighted to prioritize specific axes, yielding the regularization term $\mathrm{Trace}(\bm{D} \bm{\Psi})$, where $\bm{D}\in \real^{N_\Sigma\times N_\Sigma}$ is a diagonal matrix:
\begin{align}
	\label{eq_matrix_D}
	{\bm{D}}=
	\begin{bmatrix}
		\bm{D}_1\in \real^{N_1\times N_1}  & \cdots & 0 \\
        \vdots &  \ddots & \vdots \\
		0 & \cdots & \bm{D}_q\in \real^{N_q\times N_q}
	\end{bmatrix},
\end{align}
where $\bm{D}_i=\text{diag}\{ \bm{d}_i \}$ so that adjusting the vector $\bm{d}_i\in \real^{N_i}$ can scale the importance of compression in a certain element on the given dimension. For example, if compressing the data of $i$th dimension makes more sense due to practical constraints, one can reduce the corresponding block's diagonal in $\bm{D}$ to de-emphasize the importance of the block matrix $\tilde{\mathbf{S}}_i$ in $\bm{\Psi}$, forcing the algorithm to distribute fewer resources to this dimension.


==> sec_introduction.tex <==
\section{Introduction}\label{sec_introduction}
\begin{itemize}
    \item Multidimensional signal acquisition.
    \begin{itemize}
        \item General concept \cite{dzemyda2013multidimensional}.
        \item Concrete applications: MIMO radar\cite{li2008mimo}, MRI\cite{vlaardingerbroek2013magnetic}, FMC\cite{holmes2005post}.
    \end{itemize}
    \item Compressed sensing and subsampling.
    \begin{itemize}
        \item One sentence introduction\cite{eldar2012compressed}.
        \item Highlight subsampling is a kind of CS and its applications: \cite{lustig2007sparse,huijben2020learning, kirchhof2021frequency, nolan2024active}.
        \item Structured CS/Subsampling optimizes dimension-specific compression matrices\cite{wangicassp2024}, combining spatial\cite{wang2023deep} and Fourier\cite{perez2020subsampling} subsampling.
    \end{itemize}
    \item Task-based ML and their limitations.
    \begin{itemize}
        \item Jointly optimizing compression matrices and downstream tasks\cite{huijben2020learning, mulleti2023learning, wang2023deep}.
        \item It necessitates deep unrolled neural network\cite{monga2021algorithm} like LISTA\cite{gregor2010learning}, which is heavily-weighted in the context of large multidimensional sampling models.
        \item Despite convolutional LISTA\cite{fu2021structured, wang2024eusipco} can reduce the storage requirement, the reconstruction process still needs additional time. 
        \item Compression factor should be determined in advance in \cite{huijben2020learning, wangicassp2024}.
    \end{itemize}
    \item Motivation.
    \begin{itemize}
        \item Learning practically useful compression matrices that can be implemented in hardware.
        \item Optimize dimension-specific matrices instead of a single large compression matrix.
        \item Avoid leveraging a large network to optimize a downstream task.
        \item Automatic resource allocation.
    \end{itemize}
    \item Contributions in bullet points. 
    \begin{itemize}
        \item SCOSARA is a framework to learn dimension-specific compression matrices, we focus on subsampling matrices in this paper, which eases implementation in e.g. multistatic radar and sonar.
        \item It can optimally distribute a sampling budget across all axes.
        \item We introduce an information theory-based optimation target in this paper.
        \item We take ultrasound multichannel localization as a case study and compare it with other baseline algorithms.
    \end{itemize}
\end{itemize}

==> sec_related_work.tex <==
\section{Related Work}\label{sec_related_work}
\begin{itemize}
    \item Gumbel-Softmax trick\cite{jang2017categorical,maddison2017concrete}
    \item DPS\cite{huijben2020learning}, and adaptive DPS\cite{van2021active}
    \item J-DPS\cite{wangicassp2024}, and highlight the improvement of SCOSARA.
    \item RIP\cite{blanchard2011compressed}, FIM\cite{kay1993fundamentals}, and reconstruction\cite{ben2010cramer}. 
\end{itemize}
